FEDORA: Flying Event Dataset fOr Reactive behAvior

The ability of resource-constrained biological systems such as fruitflies to perform complex and high-speed maneuvers in cluttered environments has been one of the prime sources of inspiration for developing vision-based autonomous systems. To emulate this capability, the perception pipeline of such systems must integrate information cues from tasks including optical flow and depth estimation, object detection and tracking, and segmentation, among others. However, the conventional approach of employing slow, synchronous inputs from standard frame-based cameras constrains these perception capabilities, particularly during high-speed maneuvers. Recently, event-based sensors have emerged as low latency and low energy alternatives to standard frame-based cameras for capturing high-speed motion, effectively speeding up perception and hence navigation. For coherence, all the perception tasks must be trained on the same input data. However, present-day datasets are curated mainly for a single or a handful of tasks and are limited in the rate of the provided ground truths. To address these limitations, we present Flying Event Dataset fOr Reactive behAviour (FEDORA) - a fully synthetic dataset for perception tasks, with raw data from frame-based cameras, event-based cameras, and Inertial Measurement Units (IMU), along with ground truths for depth, pose, and optical flow at a rate much higher than existing datasets.

==> limitations.tex <==
% As explained in Section \ref{gtgen}, optical flow is computed using Eq. \ref{tran*} and \ref{flo*}. Eq. \ref{tran*} and \ref{flo*} suffer from numerical instability on and in the neighbourhood of invalid pixels. To mitigate this instability, we mark all pixels with flow values of more than a threshold value to be invalid. 
% This threshold is experimentally set to $100$.

% higher data rate, higher event rate, more complex worlds, efficient collection and storage mechanisms
While recording large sequences, the data collection and storage mechanism described in Section \ref{dataset} consumes a significant amount of dynamic memory. This makes it difficult for such sequences to be recorded on resource-constrained computer systems. The mean event rate provided by this work, as illustrated in Table \ref{seq}, while large, is still less than the event rate provided by real-world datasets such as DSEC (which provides peak event rates of $>40$ MEPS). % something more here?
We have modeled constituents of the simulation to the best of our knowledge, the difficulty and compute overhead associated with the rendering of complex physical phenomena like wind-induced swaying, intra-body interactions such as the flapping of bird wings, etc., such phenomena are absent in our simulation environment. We plan on introducing sequences from more complex environments in the future.
